Near-Optimal Collaborative Learning in Bandits

This paper introduces a general multi-agent bandit model in which each agent is facing a finite set of arms and may communicate with other agents through a central controller in order to identify, in pure exploration, or play, in regret minimization, its optimal arm. The twist is that the optimal arm for each agent is the arm with largest expected mixed reward, where the mixed reward of an arm is a weighted sum of the rewards of this arm for all agents. This makes communication between agents often necessary. This general setting allows to recover and extend several recent models for collaborative bandit learning, including the recently proposed federated learning with personalization (Shi et al., 2021). In this paper, we provide new lower bounds on the sample complexity of pure exploration and on the regret. We then propose a near-optimal algorithm for pure exploration. This algorithm is based on phased elimination with two novel ingredients: a data-dependent sampling scheme within each phase, aimed at matching a relaxation of the lower bound.

==> BAI_baselines.tex <==
\section{A Simple BAI Algorithm Inspired by PF-UCB}\label{app:pfbai_baseline}

We state below as Algorithm~\ref{algo:pfucb_bai} a straightforward adaptation of the PF-UCB algorithm in~\cite{shi2021federated} to \textit{personalized} federated 
best arm identification (BAI)~; meaning that only weight matrices of the form $w_{n,m}=\alpha \ind{(n=m)} + \frac{1-\alpha}{M}$ for any pair of agents $(n,m)$ are considered. The original regret algorithm uses phased eliminations designed for each agent to identify their best arm together with \emph{exploitation}~: when all best arms have been found, or when some agent is waiting for others to finish their own exploration rounds, agents keep playing their empirical best arm. To turn this into a $\delta$-correct BAI algorithm, we remove the exploration rounds~; keep the same sampling rule within each phase (in which the number of samples from each arm is proportional to some rate function $f(r)$)~; and calibrate the size of the confidence intervals used to perform eliminations slightly differently, introducing for any $\delta \in (0,1)$ function
\[\forall r \geq 0, B_{r}(\delta) := \sqrt{\frac{2\log\left(KM\zeta(\beta)r^{\beta}/\delta\right)}{MF(r)}}\;.\]
where $F(r) = \sum_{p=1}^{r}f(p)$, for some $\beta > 1\;.$ In practice, we use $\beta=2\;.$ 

Algorithm~\ref{algo:pfucb_bai}, that we refer to as PF-UCB-BAI, follows the same general structure as our algorithm, with the notable difference that the number of samples of an arm $k \in B_m(r)$ in phase $r$ is fixed in advance. Under PF-UCB-BAI, when arm $k$ is still in the active set $B(r)$, agent $m$ 
\begin{itemize}
 \item performs global exploration to sample it $d_{k,m}^{g}(r) := \lceil(1-\alpha) f(r)\rceil$ times
 \item and additionally performs local exploration to sample it  $d_{k,m}^{\ell}(r) := \lceil\alpha M f(r)\rceil$ extra times if furthermore $k \in B_m(r)\;.$ 
\end{itemize}
Overall, $d_{k,m}(r) := d_{k,m}^{g}(r)+d_{k,m}^{\ell}(r) = \lceil (1-\alpha) f(r)\rceil\ind(k \in B(r)) + \lceil \alpha M f(r)\rceil\ind\left(k \in B_m(r)\right)$ new samples from arm $k$ are collected by agent $m$ during phase $r$ in order to update its estimate $\hat{\mu}_{k,m}(r)$ --the average of all available $n_{k,m}(r)$ samples for arm $k$ obtained by agent $m$-- which is sent to the central server. 

%In the original algorithm, the computation of the average mean is done in the following way: each agent first computes $\hat{\mu}_{k,m}(r)$ based on its $n_{k,m}(r)$ samples, send it to the servor who does the averaging $\overline{\mu}_k(r) =\sum_{n} \overline{\mu}_{k,n}(r)$ which is sent to all players who compute their $\hat{\mu}'_{k,m}(r) = \alpha \overline{\mu}_{k,m}(r) + \alpha \overline{\mu}_k(r)$, but the servor could also send directly the $(\mu_{k,m}'(r))_{k}$ to each agent $m$.

The mixed mean of each arm $(k,m)$ can then be computed by the server as
\[\hat{\mu}_{k,m}'(r) := \left(\alpha + \frac{1-\alpha}{M}\right)\hat{\mu}_{k,m}(r) + \frac{1-\alpha}{M} \sum_{m \neq n} \hat{\mu}_{k,n}(r)\;,\]
and sent back to each agent. We note that, in~\cite{shi2021federated}, they propose that the server computes the average $\hat{\mu}_k(r) := \frac{1}{M}\sum_{m=1}^{M}\hat{\mu}_{k,m}(r)$ across agents, and sends this value to each agent, who can then obtain $\hat{\mu}_{k,m}'(r) := \alpha \hat{\mu}_{k,m}(r) + (1-\alpha)\hat{\mu}_k(r)\;.$ 

\begin{algorithm*}[t]
\caption{PF-UCB-BAI}
   \label{algo:pfucb_bai}
\begin{algorithmic}
   \STATE {\bfseries Input:} $\delta \in (0,1)$, $M$ agents, $K$ arms, matrix $W$. 
   \STATE $f(r)$: sampling effort in phase $r$, $B_r(\delta)$: size of the confidence intervals in phase $r$.
   \STATE Initialize $r \gets 0\;,$ $\forall k,m, n_{k,m}(0) \gets 0\;,$ $\forall m, B_m(0) \gets [K]\;,$ $\hat{k}_m \gets 0\;.$ %$\color{red}\hat{k}_m \gets 0$.  
   \REPEAT %\color{red}
	\STATE \textcolor{gray}{\textcolor{black}{\# Central server}}
   \IF{$|B_m(r)| = 1$}
   \STATE $\hat{k}_m \gets $ the unique arm in $B_m(r)$
   \STATE $B_m(r) = \emptyset$ 
   \ENDIF\color{black}
   \STATE $B(r) \gets \bigcup_{m \in [M]} B_m(r)$
    \FOR{$k \in B(r), m \in [M]$}
    \STATE $d_{k,m}(r) = \lceil (1-\alpha) f(r)\rceil + \lceil \alpha M f(r)\rceil\ind\left(k \in B_m(r)\right)$
    \ENDFOR
	\STATE \textcolor{black}{Send to each agent $m$ $(d_{k,m}(r))_{k,m}$ and $d_{\max} := \max_{n \in [M]} \sum_{k \in [K]} d_{k,n}(r)$}
    \STATE
	\STATE \textcolor{gray}{\textcolor{black}{\# Agent $m$}}
	\STATE Sample arm $k \in B(r)$ $d_{k,m}(r)$ times, so that $n_{k,m}(r) = n_{k,m}(r-1)+d_{k,m}(r)$
	\STATE \textcolor{black}{Remain idle for $d_{\max}-\sum_{k \in [K]} d_{k,m}(r)$ rounds}
	\STATE \textcolor{black}{Send to the server empirical mean $\hat{\mu}_{k,m}(r):=\sum_{s \leq n_{k,m}(r)} X_{k,m}(s)/n_{k,m}(r)$ for any $k \in [K]$}
    \STATE
   \STATE {\textcolor{gray}{// \emph{Update set of candidate best arms for each user}}}
   \FOR{$m=1$ {\bfseries to} $M$} 
   \STATE $B_{m}(r+1) \gets \left\{ k \in B_{m}(r) \mid \hat{\mu}'_{k,m}(r) + B_{r}(\delta) \geq \max_{j \in B_m(r)} \left( \hat{\mu}'_{j,m}(r) - B_{r}(\delta) \right) \right\}$
   \ENDFOR 
   \STATE $r \gets r+1$
   \UNTIL{$|B(r)| = \emptyset$}%{$\color{red}|B(r)| = \emptyset$}
	\STATE {\bfseries Output:} $\left\{ \hat{k}_m : m \in [M] \right\}$%$\color{red}\left\{ \hat{k}_m : m \in [M] \right\}$
\end{algorithmic}
\end{algorithm*}

Arm $k$ is eliminated from the active set $B_m(r)$ of agent $m$ if 
\[\hat{\mu}'_{k,m}(r) + B_{r}(\delta) < \max_{j \in B_m(r)} \left( \hat{\mu}'_{j,m}(r) - B_{p}(\delta) \right)\]
for the confidence parameter $B_r(\delta)$. In the original algorithm, $B_r(\delta)$ is replaced by some function of $r$ and $T$, however a simple adaptation of Lemma $1$ in~\cite{shi2021federated} (adding a union bound on $r \in \Nn$) yields the following result. Indeed, the original result crucially exploits the sampling rule, which we did not change. 

\begin{lemma}\label{lem:newlemma1} Event 
\[\mathcal{G} := \left\{\forall r \in \Nn^*, \forall m \in [M],\forall k \in B_m(r), \left|\hat{\mu}'_{k,m}(r) - \mu_{k,m}'\right|\leq B_r(\delta)\right\}\]
holds with probability $1-\delta$. 
\end{lemma}

On the good event $\mathcal{G}$ introduced in Lemma~\ref{lem:newlemma1}, observe that arm $k_m^*$ can never be eliminated from the set $B_m(r)$, therefore it has to be the guess $\hat{k}_m$ that agent $m$ outputs. This proves that Algorithm~\ref{algo:pfucb_bai} is $\delta$-correct for pure exploration for the special case of %in 
\textcolor{black}{collaborative} %federated 
bandit with personalization. %That is, for some $\alpha \in [0,1]$
%\[ W = \alpha Id_{M \times M} + \frac{1-\alpha}{M} \mathds{1}_{M \times M}\;.\]
This algorithm can therefore serve as a baseline to be compared to our proposal in this particular case. 

\textcolor{black}{
We can also upper bound the sample complexity of this algorithm. Indeed, on event $\mathcal{G}$, like in the analysis of PF-UCB in~\cite{shi2021federated}, we can upper bound the number of rounds where arm $k$ is sampled by agent $m$ by $p_{k,m} := \inf \{r : B_r(\delta) \leq  \Delta'_{k,m}/4\}$. When $f(p) = 2^p$, one can prove that 
\[ \sum_{p=1}^{p_{k,m}} f(p) = \mathcal{O}(M^{-1}(\Delta'_{k,m})^{-2}\log(1/\delta))\;. \]
Summing the (deterministic) global and local exploration cost over rounds, arms and agents, yields an exploration cost of order
\[\mathcal{O}\left( \sum_{k \in [K]} \left[ \left( \frac{1-\alpha}{\min_{n \in [M]} (\Delta'_{k,m})^2} \right) + \left( \sum_{m \in [M]} \frac{\alpha}{(\Delta'_{k,m})^2} \right) \right] \right) \;.\]
}

%\begin{comment}

%\todoe{We won't put what is below for the paper, I am just making a case that it should be sub-optimal}

%However, as it is based on deteministic exploration of active arms, we believe that the sample complexity of PF-UCB-BAI is not near-optimal, unlike that of FPE-BAI. Using similar steps of the analysis of PF-UCB for regret, we can actually establish the following sample complexity upper bound, which is not matching our lower bound.   

%\begin{theorem}\label{thm:sc_pfbai} We introduce the following quantities. For all $m$ and $k\neq k_m^*$, we let
%\[p'_{k,m}(\delta) = \inf \left\{ r \in \Nn : B_r(\delta) \leq \frac{1}{4}\Delta'_{k,m}\right\},\]
%$p'_{k_m^\star,m}(\delta) = \max_{k \neq k_m^\star} p'_{k,m}(\delta)$ and for all $k$
%\[p'_{k}(\delta) := \max_{m \in [M]} p'_{k,m}(\delta).\]
%Then, on the good event $\mathcal{G}$, the sample complexity of PF-UCB-BAI is upper bounded by 
%\[\underbrace{\sum_{k \in [K]}\sum_{m \in [M]} \sum_{r=1}^{p'_k(\delta)} \lceil(1-\alpha)f(r)}_{\text{global exploration}} \rceil +  \underbrace{\sum_{k=1}^{K}\sum_{m=1}^{M} \sum_{r=1}^{p'_{k,m}(\delta)} \lceil M\alpha f(r) \rceil}_{\text{local exploration}} \]
%\end{theorem}

%For $f(p) = 2^p$, we can certainly prove that if
%\[p_{\Delta}(\delta) := \inf \left\{ r \in \Nn : B_r(\delta) \leq \frac{1}{4}\Delta\right\}\]
%then $F(p_{\Delta}(\delta))$ is of order $\frac{C}{M\Delta^2}\log\left(\frac{KM}{\delta}\right)$ + second order terms and we will get the leading term
%\[\sum_{k=1}^{K}\sum_{m=1}^{M}\left[ \frac{(1-\alpha)}{M\min_{m} (\Delta'_{k,m})^2} + \frac{\alpha}{(\Delta'_{k,m})^2}\right] \log\left(\frac{1}{\delta}\right)\]
%in the sample complexity. 

%\todoe{(for later) if we are convinced about this sample complexity it may be worth comparing the gap-dependent constant in this leading term to $C(\mu)$...}

%\todoc{No time to understand the proof. Are you sure this works?}
%\end{comment}

%\section{Collaborative Learning}

%Remember that collaborative learning can be retrieved from our general setting for pure exploration by considering

%\[ W = Id_{M \times M} \text{ and } \forall m,n, \forall k, \mu'_{k,m} = \mu'_{k,n} = \mu_{k} \;.\]

%\todoc{Add some refs.}

%\paragraph{Lower Bound.} If we directly consider the lower bound in Theorem~\ref{thm:LBBAI}, and replace $W$ and $\mu$ accordingly, then we obtain the following lower bound for the exploration cost --remember that we do not aim at minimizing the communication cost here-- for any instance $\mu \in \Rr^{K \times M}$, $\delta \leq 1/2$, and any $\delta$-correct algorithm $\cA$ under which agents communicate after each sampling

%\[\text{Exp}_{\mu}(\cA) \geq T_C^\star(\mu) \log\left(\frac{1}{2.4\delta}\right)\;,\]

%where $T_C^\star(\mu) := \min_{t \in \Rr^{K \times M}} \sum_{(k,m) \in [K] \times [M]} t_{k,m} \text{ s.t. } \forall m, k\neq k^\star, \left(\frac{1}{t_{k,m}} + \frac{1}{t_{k^\star_m,m}}\right) \leq \frac{\left(\Delta_{k}\right)^2}{2} \;,$ and for any $m$, for any $k \neq k^\star := \arg\max_{k} \mu_k$, $\Delta_{k} := \mu_{k^\star}-\mu_{k}\;,$ and $\Delta_{k^\star} := \min_{k \neq k^\star} \Delta_{k}\;.$\\

%The bounds found in Lemma~\ref{lem:ttilde_optimal} still hold, and yield
%\[ 2M \sum_{k}1/(\Delta_k)^2 \leq T^\star_C(\mu) \leq 4M\sum_k 1/(\Delta_k)^2\;,\]

%which means this lower bound has a supplementary multiplicative factor $M$ compared to the complexity of an individual best arm identification algorithm on instance $\mu$. This can be explained by the fact that the lower bound in Theorem~\ref{thm:LBBAI} is oblivious to the fact that, in collaborative learning, different agents actually have access to the \textit{very same} distribution $\mu$.\\

%Up to some slight changes in the proof, we are able to show a tighter lower bound on the exploration cost for the specific case of collaborative learning for Gaussian bandits

%\begin{theorem}\label{thm:COLLABBAI}
%	Let $\mu$ be a fixed matrix of means in $\Rr^{K}$. For any $\delta \leq 1/2$, let $\cA$ be a $\delta$-correct \textit{collaborative learning} algorithm under which each player communicates each reward to the central server after it is observed, and let us denote for  
	%any arm $k \in [K]$ and agent $m \in [M]$, 
%	any $k$, $m$, $\tau_{k,m} := \bE_{\mu}^{\cA}\left[ N_{k,m}(\tau) \right]$, where $\tau$ is the stopping time.

% For all $m$ and $k\neq k^\star$, it holds that  
%	\[\sum_{n}w_{n,m}^2\left(\frac{1}{\tau_{k,n}} + \frac{1}{\tau_{k^\star_m,n}}\right) \geq \frac{\left(\Delta'_{k,m}\right)^2/2}{\log(1/(2.4\delta))} \;,\]
%	\todoc{I think the sign is $\geq$ instead of $\leq$, please correct me otherwise}
%and therefore $\text{Exp}_{\mu}(\cA) \geq T^\star(\mu) \log\left(\frac{1}{2.4\delta}\right)$, %where 

%\[T^\star(\mu) := \min \left\{\left.\sum_{k,m} \tau_{k,m} \right| \forall m, k\neq k^\star_m, \ \sum_{n}w_{n,m}^2\left(\frac{1}{\tau_{k,n}} + \frac{1}{\tau_{k^\star_m,n}}\right) \leq \frac{(\Delta'_{k,m})^2}{2}\right\}\;.\]

%	\begin{equation*}
%		\begin{split}
%		T^\star(\mu) := & \min_{t \in \Rr^{K \times M}} \sum_{(k,m) \in [K] \times [M]} t_{k,m} \text{ s.t. } \forall m, k\neq k^\star_m, \sum_{n \in [M]}w_{n,m}^2\left(\frac{1}{t_{k,n}} + \frac{1}{t_{k^\star_m,n}}\right) \leq \frac{\left(\Delta'_{k,m}\right)^2}{2} \;.\\ 
%		\end{split}
%	\end{equation*}
%\end{theorem}

%\begin{proof}
%	The set of alternative models to instance $\mu$ --where $k^\star(\mu) := \arg\max_{k} %\mu_k$ is assumed unique-- is
%	\[ \text{Alt}(\mu) := \{ \lambda : \exists k \neq k^\star(\mu), \lambda_{k} > %\lambda_{k^\star}\}\;.\]
%	Define event $\Ec' := \{ \forall m, \hat{k}_m = k^\star(\mu) \}$, where $\hat{k}_m$ is %the arm returned by agent $m$ in algorithm $\cA$ at (finite) stopping time $\tau$. Since $\cA$ is $\delta$-correct, then $\bP_{\mu}(\Ec') \geq 1-\delta$ and $\bP_{\lambda}(\Ec')\leq \delta$ for any alternative model $\lambda \in \text{Alt}(\mu)$. By Theorem $1$ in~\cite{garivier2016optimal}
%	\[ \frac{1}{2} \sum_{k,m} \tau_{k,m}(\mu_{k}-\lambda_{k})^2 \geq \log(1/(2.4\delta))\;. \]
%	
%\end{proof}

%Note that this lower bound is compatible with the maximal speedup for a collaborative learning algorithm on a best arm identification task, as discussed in~\cite{hillel2013distributed,tao2019collaborative}.

%\paragraph{Algorithm.}

%\todoc{TODO}


==> checklist.tex <==

% \newpage

% \section*{Checklist}

% \begin{enumerate}


% \item For all authors...
% \begin{enumerate}
%   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
%     \answerYes{}, a general framework which encompasses several prior works is described in Section~\ref{section:introduction}; a lower bound on the sample complexity for a pure exploration problem is derived in Section~\ref{sec:lower_bound_bai}, whereas a lower bound on regret on the regret minimization counterpart of the problem is shown in Section~\ref{section:regret}. An algorithm for best arm identification, using a novel approach to achieve near-optimality, is described and analyzed in Section~\ref{sec:federated_bai_algo}.
%   \item Did you describe the limitations of your work?
%     \answerYes{}, we explained that the weight matrix had to be known in advance (Section~\ref{section:introduction}), although there is an application case where it can be computed. Moreover, we explained in conclusion to our work the issue faced when applying the same technique to regret minimization (Section~\ref{sec:discussion}).
%   \item Did you discuss any potential negative societal impacts of your work?
%     \answerYes{}, we remarked in our discussion (Section~\ref{sec:discussion}) that our collaborative algorithm might not be adapted to private, sensitive data, but might still be interesting for dealing with collaborative adaptive clinical trials between trusting teams.
%   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
%     \answerYes{}
% \end{enumerate}


% \item If you are including theoretical results...
% \begin{enumerate}
%   \item Did you state the full set of assumptions of all theoretical results?
%     \answerYes{}, the assumptions are mentioned both in the statement of the results (Section~\ref{sec:lower_bound_bai}, Section~\ref{sec:federated_bai_algo}, Section~\ref{section:regret}) and the proofs (Appendix).
%         \item Did you include complete proofs of all theoretical results?
%     \answerYes{}, proofs in full are included in Appendix.
% \end{enumerate}


% \item If you ran experiments...
% \begin{enumerate}
%   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
%     \answerYes{}, the code and run traces are available in a open-source repository.~\footnote{\texttt{https://github.com/clreda/near-optimal-federated}}
%   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
%     \answerYes{}, this information is reported in Appendix~\ref{sec:experiments}.
%         \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
%     \answerYes{}, tables in Appendix~\ref{sec:experiments} reports the average values $\pm$ their standard deviation.
%         \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
%     \answerYes{}, this information is provided in Appendix~\ref{sec:experiments} (paragraph ``Numerical considerations'').
% \end{enumerate}


% \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% \begin{enumerate}
%   \item If your work uses existing assets, did you cite the creators?
%     \answerNA{}
%   \item Did you mention the license of the assets?
%   \answerNA{}
%   \item Did you include any new assets either in the supplemental material or as a URL?
%     \answerNA{}
%   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%     \answerNA{}
%   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
%     \answerNA{}
% \end{enumerate}


% \item If you used crowdsourcing or conducted research with human subjects...
% \begin{enumerate}
%   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
%     \answerNA{}
%   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
%   \answerNA{}
%   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
%   \answerNA{}
% \end{enumerate}


% \end{enumerate}
